Angle-Dependent Phase Shifter Model for Reconfigurable Intelligent Surfaces: Does the Angle-Reciprocity Hold?

The existing phase shifter models adopted for reconfigurable intelligent surfaces (RISs) have ignored the electromagnetic (EM) waves propagation behavior, thus cannot reveal practical effects of RIS on wireless communication systems. Based on the equivalent circuit, this paper introduces an angle-dependent phase shifter model for varactor-based RISs. To the best of our knowledge, this is the first phase shifter model which reveals that the incident angle of EM waves has influence on the reflection coefficient of RIS. In addition, the angle-reciprocity on RIS is investigated and further proved to be tenable when the reflection phase difference of adjacent RIS unit cells is invariant for an impinging EM wave and its reverse incident one. The angle-dependent characteristic of RIS is verified through full-wave simulation. According to our analysis and the simulation results, we find that the angle-reciprocity of varactor-based RIS only holds under small incident angles of both forward and reverse incident EM waves, thus limits the channel reciprocity in RIS-assisted TDD systems.

==> input.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Input.tex
% Last organized by Takao Inoue, March 12, 2008
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Included packages
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage{acronym}
%\usepackage{amsfonts}
%\usepackage[dvips]{graphicx}
%\usepackage{times}
%\usepackage{cite}
%\usepackage{amsmath}
%\usepackage{array}
%\usepackage{amssymb}
%\usepackage{stfloats}
%\usepackage{diagbox}
%\usepackage{graphicx}
%\usepackage{footnote}
%\usepackage{amsthm}
%\usepackage{booktabs}
%\usepackage{array}
%%\usepackage{algorithmic}
%%\usepackage{algorithm}
%\usepackage[ruled,vlined]{algorithm2e}
%\usepackage{subeqnarray}
%\usepackage{cases}
%\usepackage{threeparttable}
%\usepackage{color}
%%\usepackage{hyperref}
%\usepackage{epstopdf}
%\usepackage{multirow}
%\usepackage{tabularx}
%\usepackage{enumerate}
%\usepackage{multicol}
%\usepackage{hyperref}
%%\usepackage{subfigure}
%%\usepackage{subcaption}
%%\usepackage{subfig}
%\usepackage{subfig}
%\usepackage{caption}
%%% If you're having trouble running LaTeX to generate a DVI, comment the below.
%%% If you want to use PDF Latex and cant, try uncommenting it.
%\usepackage{graphicx}
%\usepackage{picins}
%\usepackage{wrapfig}
%\DeclareGraphicsExtensions{.pdf}


%\DeclareGraphicsExtensions{.jpg}
%\usepackage[dvips]{graphicx}
%\DeclareGraphicsExtensions{.eps}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% fancyhdr definitions (for books)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage{fancyhdr}
%\pagestyle{fancy}
%\renewcommand{\headrulewidth}{0.5pt}
%\renewcommand{\footrulewidth}{0pt}
%\newcommand{\helv}{%
%    \fontfamily{phv}\fontseries{b}\fontsize{9}{11}\selectfont}
%\fancyhf{}
%\fancyhead[LE,RO]{\helv  \thepage}
% Following should be included in each chapter's base.tex with
% appropriate chapter title.

%\fancyhead[RE]{\helv  \bfseries Advanced MIMO Communication}
%\fancyhead[LO]{\helv  \bfseries CHAPTER X. Spatial Multiplexing}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Included packages
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newtheorem{conjecture}{Conjecture}
\newtheorem{corollary}{Corollary}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{proposition}{Proposition}
\newtheorem{example}{Example}
\newtheorem{definition}{Definition}
%\newenvironment{proof}{ \textbf{Proof:} }{ \hfill $\Box$}


\newcommand{\bookemph}[1]{ {\em #1}}
%\newcommand{\comment}[1]{}
%\newcommand{\eqref}[1]{(\ref{#1})}
\newcommand{\field}[1]{\mathbb{#1}}
\newcommand{\fig}[1]{Fig.~\ref{#1}}
\newcommand{\secref}[1]{{Section}~\ref{#1}}
\newcommand{\figref}[1]{{Fig.}~\ref{#1}}
\newcommand{\tabref}[1]{{Table}~\ref{#1}}

%\renewcommand\citeform[1]{[#1]}
%\renewcommand\citeleft{}
%\renewcommand\citeright{}

\newcommand{\Ut}{U_t}
\def\onehalf{\frac{1}{2}}
\def\etal{et.\/ al.\/}
\newcommand{\bydef}{\triangleq}
\newcommand{\tr}{\it{tr}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% blackboard lowercase
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\bydef{:=}
\def\bba{{\mathbb{a}}}
\def\bbb{{\mathbb{b}}}
\def\bbc{{\mathbb{c}}}
\def\bbd{{\mathbb{d}}}
\def\bbee{{\mathbb{e}}}
\def\bbff{{\mathbb{f}}}
\def\bbg{{\mathbb{g}}}
\def\bbh{{\mathbb{h}}}
\def\bbi{{\mathbb{i}}}
\def\bbj{{\mathbb{j}}}
\def\bbk{{\mathbb{k}}}
\def\bbl{{\mathbb{l}}}
\def\bbm{{\mathbb{m}}}
\def\bbn{{\mathbb{n}}}
\def\bbo{{\mathbb{o}}}
\def\bbp{{\mathbb{p}}}
\def\bbq{{\mathbb{q}}}
\def\bbr{{\mathbb{r}}}
\def\bbs{{\mathbb{s}}}
\def\bbt{{\mathbb{t}}}
\def\bbu{{\mathbb{u}}}
\def\bbv{{\mathbb{v}}}
\def\bbw{{\mathbb{w}}}
\def\bbx{{\mathbb{x}}}
\def\bby{{\mathbb{y}}}
\def\bbz{{\mathbb{z}}}
\def\bb0{{\mathbb{0}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Bold lowercase
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\bydef{:=}
\def\ba{{\mathbf{a}}}
\def\bb{{\mathbf{b}}}
\def\bc{{\mathbf{c}}}
\def\bd{{\mathbf{d}}}
\def\bee{{\mathbf{e}}}
\def\bff{{\mathbf{f}}}
\def\bg{{\mathbf{g}}}
\def\bh{{\mathbf{h}}}
\def\bi{{\mathbf{i}}}
\def\bj{{\mathbf{j}}}
\def\bk{{\mathbf{k}}}
\def\bl{{\mathbf{l}}}
\def\bm{{\mathbf{m}}}
\def\bn{{\mathbf{n}}}
\def\bo{{\mathbf{o}}}
\def\bp{{\mathbf{p}}}
\def\bq{{\mathbf{q}}}
\def\br{{\mathbf{r}}}
\def\bs{{\mathbf{s}}}
\def\bt{{\mathbf{t}}}
\def\bu{{\mathbf{u}}}
\def\bv{{\mathbf{v}}}
\def\bw{{\mathbf{w}}}
\def\bx{{\mathbf{x}}}
\def\by{{\mathbf{y}}}
\def\bz{{\mathbf{z}}}
\def\b0{{\mathbf{0}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Bold capital letters
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\bA{{\mathbf{A}}}
\def\bB{{\mathbf{B}}}
\def\bC{{\mathbf{C}}}
\def\bD{{\mathbf{D}}}
\def\bE{{\mathbf{E}}}
\def\bF{{\mathbf{F}}}
\def\bG{{\mathbf{G}}}
\def\bH{{\mathbf{H}}}
\def\bI{{\mathbf{I}}}
\def\bJ{{\mathbf{J}}}
\def\bK{{\mathbf{K}}}
\def\bL{{\mathbf{L}}}
\def\bM{{\mathbf{M}}}
\def\bN{{\mathbf{N}}}
\def\bO{{\mathbf{O}}}
\def\bP{{\mathbf{P}}}
\def\bQ{{\mathbf{Q}}}
\def\bR{{\mathbf{R}}}
\def\bS{{\mathbf{S}}}
\def\bT{{\mathbf{T}}}
\def\bU{{\mathbf{U}}}
\def\bV{{\mathbf{V}}}
\def\bW{{\mathbf{W}}}
\def\bX{{\mathbf{X}}}
\def\bY{{\mathbf{Y}}}
\def\bZ{{\mathbf{Z}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Blackboard capital letters
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\bbA{{\mathbb{A}}}
\def\bbB{{\mathbb{B}}}
\def\bbC{{\mathbb{C}}}
\def\bbD{{\mathbb{D}}}
\def\bbE{{\mathbb{E}}}
\def\bbF{{\mathbb{F}}}
\def\bbG{{\mathbb{G}}}
\def\bbH{{\mathbb{H}}}
\def\bbI{{\mathbb{I}}}
\def\bbJ{{\mathbb{J}}}
\def\bbK{{\mathbb{K}}}
\def\bbL{{\mathbb{L}}}
\def\bbM{{\mathbb{M}}}
\def\bbN{{\mathbb{N}}}
\def\bbO{{\mathbb{O}}}
\def\bbP{{\mathbb{P}}}
\def\bbQ{{\mathbb{Q}}}
\def\bbR{{\mathbb{R}}}
\def\bbS{{\mathbb{S}}}
\def\bbT{{\mathbb{T}}}
\def\bbU{{\mathbb{U}}}
\def\bbV{{\mathbb{V}}}
\def\bbW{{\mathbb{W}}}
\def\bbX{{\mathbb{X}}}
\def\bbY{{\mathbb{Y}}}
\def\bbZ{{\mathbb{Z}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Caligraphic capital letters
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Sans serif capital letters
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\sfA{\mathsf{A}}
\def\sfB{\mathsf{B}}
\def\sfC{\mathsf{C}}
\def\sfD{\mathsf{D}}
\def\sfE{\mathsf{E}}
\def\sfF{\mathsf{F}}
\def\sfG{\mathsf{G}}
\def\sfH{\mathsf{H}}
\def\sfI{\mathsf{I}}
\def\sfJ{\mathsf{J}}
\def\sfK{\mathsf{K}}
\def\sfL{\mathsf{L}}
\def\sfM{\mathsf{M}}
\def\sfN{\mathsf{N}}
\def\sfO{\mathsf{O}}
\def\sfP{\mathsf{P}}
\def\sfQ{\mathsf{Q}}
\def\sfR{\mathsf{R}}
\def\sfS{\mathsf{S}}
\def\sfT{\mathsf{T}}
\def\sfU{\mathsf{U}}
\def\sfV{\mathsf{V}}
\def\sfW{\mathsf{W}}
\def\sfX{\mathsf{X}}
\def\sfY{\mathsf{Y}}
\def\sfZ{\mathsf{Z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sans serif lowercase
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\bydef{:=}
\def\sfa{{\mathsf{a}}}
\def\sfb{{\mathsf{b}}}
\def\sfc{{\mathsf{c}}}
\def\sfd{{\mathsf{d}}}
\def\sfee{{\mathsf{e}}}
\def\sfff{{\mathsf{f}}}
\def\sfg{{\mathsf{g}}}
\def\sfh{{\mathsf{h}}}
\def\sfi{{\mathsf{i}}}
\def\sfj{{\mathsf{j}}}
\def\sfk{{\mathsf{k}}}
\def\sfl{{\mathsf{l}}}
\def\sfm{{\mathsf{m}}}
\def\sfn{{\mathsf{n}}}
\def\sfo{{\mathsf{o}}}
\def\sfp{{\mathsf{p}}}
\def\sfq{{\mathsf{q}}}
\def\sfr{{\mathsf{r}}}
\def\sfs{{\mathsf{s}}}
\def\sft{{\mathsf{t}}}
\def\sfu{{\mathsf{u}}}
\def\sfv{{\mathsf{v}}}
\def\sfw{{\mathsf{w}}}
\def\sfx{{\mathsf{x}}}
\def\sfy{{\mathsf{y}}}
\def\sfz{{\mathsf{z}}}
\def\sf0{{\mathsf{0}}}




% R M capital letters
\def\rmA{\mathrm{A}}
\def\rmB{\mathrm{B}}
\def\rmC{\mathrm{C}}
\def\rmD{\mathrm{D}}
\def\rmE{\mathrm{E}}
\def\rmF{\mathrm{F}}
\def\rmG{\mathrm{G}}
\def\rmH{\mathrm{H}}
\def\rmI{\mathrm{I}}
\def\rmJ{\mathrm{J}}
\def\rmK{\mathrm{K}}
\def\rmL{\mathrm{L}}
\def\rmM{\mathrm{M}}
\def\rmN{\mathrm{N}}
\def\rmO{\mathrm{O}}
\def\rmP{\mathrm{P}}
\def\rmQ{\mathrm{Q}}
\def\rmR{\mathrm{R}}
\def\rmS{\mathrm{S}}
\def\rmT{\mathrm{T}}
\def\rmU{\mathrm{U}}
\def\rmV{\mathrm{V}}
\def\rmW{\mathrm{W}}
\def\rmX{\mathrm{X}}
\def\rmY{\mathrm{Y}}
\def\rmZ{\mathrm{Z}}
\def\sign{{\mathrm{sign}}}

% R M lowercase
\def\bydef{:=}
\def\rma{{\mathrm{a}}}
\def\rmb{{\mathrm{b}}}
\def\rmc{{\mathrm{c}}}
\def\rmd{{\mathrm{d}}}
\def\rmee{{\mathrm{e}}}
\def\rmff{{\mathrm{f}}}
\def\rmg{{\mathrm{g}}}
\def\rmh{{\mathrm{h}}}
\def\rmi{{\mathrm{i}}}
\def\rmj{{\mathrm{j}}}
\def\rmk{{\mathrm{k}}}
\def\rml{{\mathrm{l}}}
\def\rmm{{\mathrm{m}}}
\def\rmn{{\mathrm{n}}}
\def\rmo{{\mathrm{o}}}
\def\rmp{{\mathrm{p}}}
\def\rmq{{\mathrm{q}}}
\def\rmr{{\mathrm{r}}}
\def\rms{{\mathrm{s}}}
\def\rmt{{\mathrm{t}}}
\def\rmu{{\mathrm{u}}}
\def\rmv{{\mathrm{v}}}
\def\rmw{{\mathrm{w}}}
\def\rmx{{\mathrm{x}}}
\def\rmy{{\mathrm{y}}}
\def\rmz{{\mathrm{z}}}
\def\rm0{{\mathrm{0}}}


\def\Nt{{N_\mathrm{T}}}
\def\Nta{{N_\mathrm{t}^{\mathrm{a}}}}
\def\Nte{{N_\mathrm{t}^{\mathrm{e}}}}
\def\Nr{{N_\mathrm{R}}}
\def\Nra{{N_\mathrm{r}^{\mathrm{a}}}}
\def\Nre{{N_\mathrm{r}^{\mathrm{e}}}}
\def\Np{{N_\mathrm{p}}}
\def\Nb{{N_\mathrm{b}}}
\def\Nc{{N_\mathrm{c}}}
\def\Ncl{{N_\mathrm{cl}}}
\def\Nct{{N_{\mathrm{t}}}}
\def\Ncr{{N_{\mathrm{r}}}}
\def\Ns{{N_\mathrm{s}}}
\def\Ne{{N_e}}
\def\Es{{E_s}}
\def\No{{N_o}}
\def\sinc{\mathrm{sinc}}
\def\dmin{d^2_{\mathrm{min}}}
\def\vec{\mathrm{vec}~}
\def\kron{\otimes}
\def\Pe{{P_e}}
\def\Pt{{P_{\mr{t}}}}
\def\Hb{{\mathcal{H}_{\mr{b}}}}

% Added by Takao
\def\nn{\nonumber}

% Chapter Numbers
\def\IntroChapter{Chapter 1 }
\def\SPChapter{Chapter 2 }
\def\ChanChapter{Chapter 3 }
\def\ITChapter{Chapter 4 }
\def\CTChapter{Chapter 5 }
\def\SMChapter{Chapter 6 }
\def\STCChapter{Chapter 7 }
\def\SULFChapter{Chapter 8 }
\def\MUITChapter{Chapter 9 }
\def\MUMIMOChapter{Chapter 10 }
\def\MULFChapter{Chapter 11 }
\def\LAChapter{Chapter 12 }
\def\MIMONetworksChapter{Chapter 13 }
\def\MIMOantChapter{Chapter 14 }
\def\PracticalChapter{Chapter 15 }
\def\StandardN{Chapter 16 }
\def\StandardE{Chapter 17 }
\def\StandardGPP{Chapter 18 }


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Robert's Notation Commands - Just temporary
\newcommand{\signb}{s} % not bold
\newcommand{\sig}{\mathbf{s}}
\newcommand{\Sig}{\mathbf{S}}
\newcommand{\noise}{\mathbf{v}}
\newcommand{\noisenb}{v}
\newcommand{\data}{\mathbf{y}}
\newcommand{\datanb}{{y}}
\newcommand{\Ff}{\mathsf{F}}
\newcommand{\ff}{\mathsf{f}}
\newcommand{\Hf}{\mathsf{H}}
\newcommand{\Gf}{\mathsf{G}}
\newcommand{\Ht}{\mathbf{H}}
\newcommand{\htime}{h}
\newcommand{\hfreq}{H}
\newcommand{\ftime}{f}
\newcommand{\ffreq}{F}
\newcommand{\Mt}{M_t}
\newcommand{\Mr}{M_r}
\newcommand{\evec}{\mathbf{e}}
\newcommand{\chanvec}{\mathbf{h}}
\newcommand{\symvecset}{\mathcal{S}}

%%%% Antonio's add %%%%%%%%%%%%%%%%%%%
\newcommand{\bLam}{\mathbf{\Lambda}}
\newcommand{\defeq}{\bydef}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%% Jianhua Mo's add %%%%%%%%%%%%%%%%%%%
\newcommand{\mb}{\mathbf}
\newcommand{\mr}{\mathrm}
\def\j{\mathrm{j}}
\def\Re{\mathrm{Re}}
\def\Im{\mathrm{Im}}
\acrodef{CSI}[CSI]{channel state information}
\acrodef{CSIT}[CSIT]{channel state information at the transmitter}
\acrodef{CSIR}[CSIR]{channel state information at the receiver}
\acrodef{MIMO}[MIMO]{multiple-input multiple-output}
\acrodef{SISO}[SISO]{single-input single-output}
\acrodef{MISO}[MISO]{multiple-input single-output}
\acrodef{SIMO}[SIMO]{single-input multiple-output}
\acrodef{ADCs}[ADCs]{analog-to-digital convertors}
\acrodef{SNR}[SNR]{signal-to-noise ratio}
\acrodef{AWGN}[AWGN]{additive white Gaussian noise}
\acrodef{MRT}[MRT]{maximal ratio transmission}
\acrodef{DFT}[DFT]{Discrete Fourier Transform}
\acrodef{ULA}[ULA]{uniform linear array}
\acrodef{UPA}[UPA]{uniform planar array}
\acrodef{LS}[LS]{least squares}
\acrodef{ALMMSE}[ALMMSE]{approximate linear minimum mean squared error}
\acrodef{QIHT}[QIHT]{quantized iterative hard thresholding}
\acrodef{QIST}[QIST]{quantized iterative soft thresholding}
\acrodef{SVD}[SVD]{singular value decomposition}


==> macro.TeX <==


    %\newcommand{\tr}{\mbox{trace}}
    \def\bm#1{\boldsymbol{#1}}
    \def\ang#1{\mbox{$\langle #1 \rangle$}}
    \def\aang#1{\mbox{$\langle\!\langle #1 \rangle\!\rangle$}}

    \def\mnorm#1{\mbox{$\left|\!\left|\!\left|\, #1 \,\right|\!\right|\!\right|$}}



    \def\Complex{{\rm\rule[.23ex]{.03em}{1.1ex}\kern-.3em{C}}}
    \def\bms#1{\mbox{\boldmath $\scriptstyle #1$}}
    \def\eqover#1{\mbox{$\buildrel #1 \over =$}}
    \def\leqover#1{\mbox{$\buildrel #1 \over \leq$}}
    \def\Imag#1{\mbox{${\Im}\left\{ #1 \right\}$}}
    \def\dist{\mbox{${\sf dist}(z, {\mathbb R}^+)$}}
    \def\largeN{\mbox{${\cal N}$}}

    \newcommand{\be}{\begin{equation}} \newcommand{\ee}{\end{equation}}
    \newcommand{\bea}{\begin{eqnarray}} \newcommand{\eea}{\end{eqnarray}}
    \newcommand{\benum}{\begin{enumerate}} \newcommand{\eenum}{\end{enumerate}}
    \def\proof{\noindent\hspace{2em}{\itshape Proof: }}
    \def\aproof{\noindent\hspace{2em}{\itshape Alternative Proof: }}
    \def\endproof{\hspace*{\fill}~$\square$\par\endtrivlist\unskip}
    \def\endaproof{\hspace*{\fill}~$\square$\par\endtrivlist\unskip}

  %\newtheorem{theorem}{Theorem}
  %\newtheorem{conjecture}{Conjecture}
  %\newtheorem{definition}{Definition}
  %\newtheorem{example}{Example}
  %\newtheorem{lemma}{Lemma}
  %\newtheorem{proposition}{Proposition}
  %\newtheorem{claim}{Claim}

  \def \veclen {0.8}
  \def \uppos{1.2}
  \def \lowpos{-1.5}
  \def \recwid{0.6}
  \def \rechig{0.4}
  \def \crad{0.25}

  \def \Fwid{0.8}

  \newcommand{\tbox}[1]{%

     \bsegment
      \realmult {\rechig}{0.5} \ta
      \realmult {\recwid}{0.5} \tb
       \lvec (0 \ta)    \lvec ({\recwid} \ta)
       \lvec ({\recwid} -\ta) \lvec (0 -\ta)\lvec (0 0)
       \textref h:C v:C \htext ({\tb} 0){#1}
       \savepos ({\recwid} 0)(*ex *ey)
     \esegment
     \move (*ex *ey)}

  \newcommand{\tcir}[1]{%
     \bsegment
     \realmult {\crad}{2} \ta
       \move({\crad} 0)
       \lcir r:{\crad}
       \textref h:C v:C \htext ({\crad} 0) {#1}
       \savepos ({\ta} 0)(*ex *ey)
     \esegment
     \move (*ex *ey)}


  \newcommand{\tupnoisec}[1]{%
     \bsegment
     \realadd{\crad}{0.35}\arrowlen
     \realadd{\arrowlen}{0.08}\txtpos
     \rmove({-\crad} \arrowlen) \avec({-\crad} \crad)
     \textref h:C v:C \htext ({-\crad} \txtpos){#1}
     \esegment}

    %%%%%% DEFINITION %%%%%%%%%%%%%%
    \newcommand{\qa}{{\bf a}}
    \newcommand{\qb}{{\bf b}}
    \newcommand{\qc}{{\bf c}}
    \newcommand{\qd}{{\bf d}}
    \newcommand{\qe}{{\bf e}}
    \newcommand{\qf}{{\bf f}}
    \newcommand{\qg}{{\bf g}}
    \newcommand{\qh}{{\bf h}}
    \newcommand{\qi}{{\bf i}}
    \newcommand{\qj}{{\bf j}}
    \newcommand{\qk}{{\bf k}}
    \newcommand{\ql}{{\bf l}}
    \newcommand{\qm}{{\bf m}}
    \newcommand{\qn}{{\bf n}}
    \newcommand{\qo}{{\bf o}}
    \newcommand{\qp}{{\bf p}}
    \newcommand{\qq}{{\bf q}}
    \newcommand{\qr}{{\bf r}}
    \newcommand{\qs}{{\bf s}}
    \newcommand{\qt}{{\bf t}}
    \newcommand{\qu}{{\bf u}}
    \newcommand{\qv}{{\bf v}}
    \newcommand{\qw}{{\bf w}}
    \newcommand{\qx}{{\bf x}}
    \newcommand{\qy}{{\bf y}}
    \newcommand{\qz}{{\bf z}}

    \newcommand{\qA}{{\bf A}}
    \newcommand{\qB}{{\bf B}}
    \newcommand{\qC}{{\bf C}}
    \newcommand{\qD}{{\bf D}}
    \newcommand{\qE}{{\bf E}}
    \newcommand{\qF}{{\bf F}}
    \newcommand{\qG}{{\bf G}}
    \newcommand{\qH}{{\bf H}}
    \newcommand{\qI}{{\bf I}}
    \newcommand{\qJ}{{\bf J}}
    \newcommand{\qK}{{\bf K}}
    \newcommand{\qL}{{\bf L}}
    \newcommand{\qM}{{\bf M}}
    \newcommand{\qN}{{\bf N}}
    \newcommand{\qO}{{\bf O}}
    \newcommand{\qP}{{\bf P}}
    \newcommand{\qQ}{{\bf Q}}
    \newcommand{\qR}{{\bf R}}
    \newcommand{\qS}{{\bf S}}
    \newcommand{\qT}{{\bf T}}
    \newcommand{\qU}{{\bf U}}
    \newcommand{\qV}{{\bf V}}
    \newcommand{\qW}{{\bf W}}
    \newcommand{\qX}{{\bf X}}
    \newcommand{\qY}{{\bf Y}}
    \newcommand{\qZ}{{\bf Z}}
    \newcommand{\qzero}{{\bf 0}}
    \newcommand{\qone}{{\bf 1}}
    \newcommand{\qdh}{\triangle\qh}
    \newcommand{\qhh}{\hat\qh}
    \newcommand{\qdH}{\triangle\qH}
    \newcommand{\qhH}{\hat\qH}
    \newcommand{\qdF}{\triangle\qF}
    \newcommand{\qhF}{\hat\qF}
    \newcommand{\qbh}{\bar\qh}
    \newcommand{\qbn}{\bar\qn}

    \newcommand{\qwbE}{\overline{\bf E}}
    \newcommand{\qwbF}{\overline{\bf F}}
    \newcommand{\qwbT}{\overline{\bf T}}
    \newcommand{\qwbR}{\overline{\bf R}}

    \newcommand{\qDelta}{{\boldsymbol \Delta}}
    \newcommand{\qPsi}{{\boldsymbol \Psi}}
    \newcommand{\qPhi}{{\boldsymbol \Phi}}
    \newcommand{\qXi}{{\boldsymbol \Xi}}
    \newcommand{\qTheta}{{\boldsymbol \Theta}}
    \newcommand{\qLambda}{{\boldsymbol \Lambda}}
    \newcommand{\qSigma}{{\boldsymbol \Sigma}}
    \newcommand{\qGamma}{{\boldsymbol \Gamma}}
    \newcommand{\qUpsilon}{{\boldsymbol \Upsilon}}
    \newcommand{\qOmega}{{\boldsymbol \Omega}}
    \newcommand{\qPi}{{\boldsymbol \Pi}}

    \newcommand{\qalpha}{{\boldsymbol \alpha}}
    \newcommand{\qbeta}{{\boldsymbol \beta}}
    \newcommand{\qdelta}{{\boldsymbol \delta}}
    \newcommand{\qlambda}{{\boldsymbol \lambda}}
    \newcommand{\qgamma}{{\boldsymbol \gamma}}
    \newcommand{\qepsilon}{{\boldsymbol \epsilon}}
    \newcommand{\qeta}{{\boldsymbol \eta}}
    \newcommand{\qnu}{{\boldsymbol \nu}}
    \newcommand{\qmu}{{\boldsymbol \mu}}
    \newcommand{\qkappa}{{\boldsymbol \kappa}}
    \newcommand{\qtau}{{\boldsymbol \tau}}
    \newcommand{\qxi}{{\boldsymbol \xi}}
    \newcommand{\qzeta}{{\boldsymbol \zeta}}
    \newcommand{\qvarepsilon}{{\boldsymbol \varepsilon}}
    \newcommand{\qomega}{{\boldsymbol \omega}}

    \newcommand{\tH}{{\tilde{H}}}
    \newcommand{\tQ}{{\tilde{Q}}}
    \newcommand{\talpha}{{\tilde{\alpha}}}
    \newcommand{\ttau}{{\tilde{\tau}}}

    \newcommand{\tb}{{\tilde{b}}}
    \newcommand{\tc}{{\tilde{c}}}
    \newcommand{\te}{{\tilde{e}}}
    \newcommand{\tm}{{\tilde{m}}}
    \newcommand{\tq}{{\tilde{q}}}
    \newcommand{\tv}{{\tilde{v}}}
    \newcommand{\trho}{{\tilde{\rho}}}
    \newcommand{\tvarepsilon}{{\tilde{\varepsilon}}}

    \newcommand{\tqh}{{\tilde{\qh}}}
    \newcommand{\tqv}{{\tilde{\qv}}}
    \newcommand{\tqH}{{\tilde{\qH}}}
    \newcommand{\tqU}{{\tilde{\qU}}}
    \newcommand{\tqV}{{\tilde{\qV}}}
    \newcommand{\tqD}{{\tilde{\qD}}}
    \newcommand{\tqQ}{{\tilde{\qQ}}}
    \newcommand{\tchi}{{\tilde{\chi}}}
    \newcommand{\tqTheta}{{\tilde{\qTheta}}}
    \newcommand{\tqDelta}{{\tilde{\qDelta}}}
    \newcommand{\tqPsi}{{\tilde{\qPsi}}}
    \newcommand{\tqPhi}{{\tilde{\qPhi}}}
    \newcommand{\tcalqS}{{\tilde{\calqS}}}
    \newcommand{\tqXi}{{\tilde{\qXi}}}

    \newcommand{\tqLambda}{{\tilde{\qLambda}}}

    \newcommand{\hQ}{{\hat{Q}}}

    %\newcommand{\hm}{{\hat{m}}}
    \newcommand{\hchi}{{\hat{\chi}}}

    \newcommand{\hr}{{\hat{r}}}
    \newcommand{\hs}{{\hat{s}}}
    \newcommand{\hq}{{\hat{q}}}
    \newcommand{\hp}{{\hat{p}}}
    \newcommand{\bp}{{\bar{p}}}
    \newcommand{\bv}{{\bar{v}}}
    \newcommand{\bH}{{\bar{H}}}
    \newcommand{\bqH}{{\bar{\qH}}}

    \newcommand{\whqX}{{\widehat{\qX}}}
    \newcommand{\whqZ}{{\widehat{\qZ}}}
    \newcommand{\whqH}{{\widehat{\qH}}}
    \newcommand{\whX}{{\widehat{X}}}
    \newcommand{\whH}{{\widehat{H}}}
    \newcommand{\whZ}{{\widehat{Z}}}

    \newcommand{\wtqY}{{\widetilde{\qY}}}
    \newcommand{\wtY}{{\widetilde{Y}}}
    \newcommand{\wty}{{\widetilde{y}}}


    \newcommand{\uqB}{{\underline{\qB}}}
    \newcommand{\uH}{{\underline{H}}}
    \newcommand{\utH}{{\underline{\tH}}}
    \newcommand{\ubH}{{\underline{\bH}}}
    \newcommand{\uR}{{\underline{R}}}
    \newcommand{\uT}{{\underline{T}}}
    \newcommand{\uqH}{{\underline{\qH}}}
    \newcommand{\uqR}{{\underline{\qR}}}
    \newcommand{\uqT}{{\underline{\qT}}}
    \newcommand{\ubqH}{{\underline{\bqH}}}
    \newcommand{\utqH}{{\underline{\tqH}}}
    \newcommand{\ucalqX}{{\underline{\calqX}}}
    \newcommand{\uqX}{{\underline{\qX}}}

    \newcommand{\bbB}{{\mathbb B}}
    \newcommand{\bbE}{{\mathbb E}}
    \newcommand{\bbN}{{\mathbb N}}
    \newcommand{\bbR}{{\mathbb R}}
    \newcommand{\bbC}{{\mathbb C}}
    \newcommand{\bbS}{{\mathbb S}}
    \newcommand{\bbU}{{\mathbb U}}
    \newcommand{\bbQ}{{\mathbb Q}}

    \newcommand{\calA}{{\mathcal A}}
    \newcommand{\calB}{{\mathcal B}}
    \newcommand{\calC}{{\mathcal C}}
    \newcommand{\calD}{{\mathcal D}}
    \newcommand{\calE}{{\mathcal E}}
    \newcommand{\calF}{{\mathcal F}}
    \newcommand{\calG}{{\mathcal G}}
    \newcommand{\calI}{{\mathcal I}}
    \newcommand{\calK}{{\mathcal K}}
    \newcommand{\calL}{{\mathcal L}}
    \newcommand{\calM}{{\mathcal M}}
    \newcommand{\calN}{{\mathcal N}}
    \newcommand{\calS}{{\mathcal S}}
    \newcommand{\calT}{{\mathcal T}}
    \newcommand{\calO}{{\mathcal O}}
    \newcommand{\calQ}{{\mathcal Q}}
    \newcommand{\calR}{{\mathcal R}}
    \newcommand{\calV}{{\mathcal V}}
    \newcommand{\calX}{{\mathcal X}}

    \newcommand{\calqA}{\boldsymbol{\cal A}}
    \newcommand{\calqB}{\boldsymbol{\cal B}}
    \newcommand{\calqH}{\boldsymbol{\cal H}}
    \newcommand{\calqX}{\boldsymbol{\cal X}}
    \newcommand{\calqQ}{\boldsymbol{\cal Q}}
    \newcommand{\calqS}{\boldsymbol{\cal S}}
    \newcommand{\calqZ}{\boldsymbol{\cal Z}}



    \newcommand{\dom}{{\sf dom}}
    \newcommand{\epi}{{\sf epi}}
    \newcommand{\diag}{{\sf diag}}
    \newcommand{\supp}{{\sf supp}}
    \newcommand{\tr}{{\sf tr}}
    \newcommand{\Ex}{{\sf E}}
    \newcommand{\rank}{{\sf rank}}
    \newcommand{\Varx}{{\sf Var}}
    \newcommand{\Extr}{\operatornamewithlimits{\sf Extr}}
    \newcommand{\mmse}{{\sf mmse}}
    \newcommand{\mse}{{\sf mse}}
    \newcommand{\vect}{{\sf vec}}
    \newcommand*{\argmin}{\operatornamewithlimits{argmin}\limits}
    \newcommand*{\argmax}{\operatornamewithlimits{argmax}\limits}
    \newcommand{\sfQ}{{\sf Q}}
    \newcommand{\sign}{{\sf sign}}


    \newcommand{\rmd}{{\rm d}}
    \newcommand{\rmD}{{\rm D}}

    \newcommand{\sfa}{{\sf a}}
    \newcommand{\sfb}{{\sf b}}
    \newcommand{\sfc}{{\sf c}}
    \newcommand{\sfd}{{\sf d}}
    \newcommand{\sfe}{{\sf e}}
    \newcommand{\sff}{{\sf f}}
    \newcommand{\sfg}{{\sf g}}
    \newcommand{\sfh}{{\sf h}}
    \newcommand{\sfi}{{\sf i}}
    \newcommand{\sfj}{{\sf j}}
    \newcommand{\sfk}{{\sf k}}
    \newcommand{\sfl}{{\sf l}}
    \newcommand{\sfm}{{\sf m}}
    \newcommand{\sfn}{{\sf n}}
    \newcommand{\sfo}{{\sf o}}
    \newcommand{\sfp}{{\sf p}}
    \newcommand{\sfq}{{\sf q}}
    \newcommand{\sfr}{{\sf r}}
    \newcommand{\sfs}{{\sf s}}
    \newcommand{\sft}{{\sf t}}
    \newcommand{\sfu}{{\sf u}}
    \newcommand{\sfv}{{\sf v}}
    \newcommand{\sfw}{{\sf w}}
    \newcommand{\sfx}{{\sf x}}
    \newcommand{\sfy}{{\sf y}}
    \newcommand{\sfz}{{\sf z}}




    \newcommand{\sfB}{{\sf B}}
    \newcommand{\sfC}{{\sf C}}
    \newcommand{\sfF}{{\sf F}}
    \newcommand{\sfH}{{\sf H}}
    \newcommand{\sfP}{{\sf P}}
    \newcommand{\sfX}{{\sf X}}
    \newcommand{\sfZ}{{\sf Z}}
    \newcommand{\sfqB}{\boldsymbol{\sf B}}
    \newcommand{\sfqH}{\boldsymbol{\sf H}}
    \newcommand{\sfqX}{\boldsymbol{\sf X}}
    \newcommand{\sfqx}{\boldsymbol{\sf x}}
    \newcommand{\sfqh}{\boldsymbol{\sf h}}

    \newcommand{\scP}{\mathscr{P}}
    \newcommand{\scF}{\mathscr{F}}

    \newcommand{\aaa}{\buildrel{\circ}\over{a}}
    \newcommand{\aag}{\buildrel{\circ}\over{g}}
    \newcommand{\aeta}{\buildrel{\circ}\over{\eta}}
    \newcommand{\arho}{\buildrel{\circ}\over{\rho}}
    \newcommand{\aalpha}{\buildrel{\circ}\over{\alpha}}
    \newcommand{\ateta}{\buildrel{\circ}\over{\tilde\eta}}
    \newcommand{\atalpha}{\buildrel{\circ}\over{\tilde\alpha}}
    \newcommand{\atrho}{\buildrel{\circ}\over{\tilde\rho}}


    \newcommand{\bfbl}[1]{\bf \color{blue}#1}
    \newcommand{\bl}[1]{\color{blue}#1}
    \newcommand{\bfrl}[1]{\bf \color{red}#1}
    \newcommand{\rl}[1]{\color{red}#1}
    \newcommand{\bfbrl}[1]{\bf \color{BrickRed}#1}
    \newcommand{\bfbbl}[1]{\bf \color{BlueViolet}#1}




    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

